Optimal Azimuth Sampling and Interpolation for Bistatic ISAC Setups

A key challenge in future 6G Integrated Sensing and Communications (ISAC) networks is to define the angular operations of transmitter and receiver, i.e., the sampling task of the angular domains, to acquire information about the environment. In this work we extend previous analysis for optimal angular sampling of monostatic setups to two-dimensional bistatic deployments, that are as important as the former in future ISAC cellular scenarios. Our approach overcomes the limitations of suboptimal prior art sampling and interpolation techniques, such as spline interpolation. We demonstrate that separating azimuth operations of the two transmit and receive arrays is optimal to sample the angular domain in an array-specific normalized angular frequency (NAF). This allows us to derive a loss-less reconstruction of the angular domain, enabling a more efficient and accurate sampling strategy for bistatic sensing applications compared to legacy approaches. As demonstrated by different Monte Carlo experiments, our approach enables future bistatic ISAC deployments with better performance compared to the other suboptimal solutions.

==> Figures/Cartesian/X_sweep_same_y/f1_score.tex <==
\begin{tikzpicture}

% \def\scale{.72}  % .72

\begin{semilogyaxis}[
    xlabel={$\mu^{\text{(x)}}$ [m]},
    ylabel={$F_1$},
    % ylabel shift = -14pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.02,.5)},rotate=0,anchor=south},
    x label style={yshift=0.3em},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 2, 3, 4, 5, 6},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , ,$10^{-2}$, , , , , , , , , $10^{-1}$ , , , , , , , , , $10^{0}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=2pt},  % xshift=3pt
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=5e-1,
    ymax=1e-0,
    xmin=-20,
    xmax=20,
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    % legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    % legend columns = 8,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend cell align={left},
    legend columns = 4,
    legend style={
      fill opacity=1.0,
      draw opacity=1,
      text opacity=1,
      at={(0.999,0.999)},  % single col: (0.275,0.03) original: (0.91,0.86)
      anchor=north east,
      draw=lightgray,
      font=\scriptsize
    },
    % legend style={
    % cells={anchor=west},
    % % draw=none,
    % fill=none,
    % font=\footnotesize
    % },
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    width=\figwidth,
    height=\figheight,
    scale = \scale
]


% % legend / single row
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(N^{(\text{s},\text{1D})}\)}
% \addplot[very thick, color=violet, solid] coordinates {(0, 1)}; \addlegendentry{\(3\)\hspace{-.5cm}}
% \addplot[very thick, color=teal, solid] coordinates {(0, 1)}; \addlegendentry{\(5\)}
% \addplot[very thick, color=cyan, solid] coordinates {(0, 1)}; \addlegendentry{\(7\)}
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(d^{(\text{s})}\)}
% \addplot[very thick, color=black, solid] coordinates {(0, 1)}; \addlegendentry{\( \lambda/2\)}
% \addplot[very thick, color=black, dashed] coordinates {(0, 1)}; \addlegendentry{\( 3\lambda/2\)}
% \addplot[very thick, color=black, dotted] coordinates {(0, 1)};\addlegendentry{\(2 \lambda\)}


\def\dirstr{"Cartesian/X_sweep_same_y"}
\def\evalstr{"f1_score"}

\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr.txt};
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr_baseline.txt};
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr_baseline_rad.txt};


\end{semilogyaxis}

\end{tikzpicture}


==> Figures/Cartesian/X_sweep_same_y/fa_rate.tex <==
\begin{tikzpicture}

% \def\scale{.72}  % .72

\begin{semilogyaxis}[
    xlabel={$\mu^{\text{(x)}}$ [m]},
    ylabel={$R^\text{(FA)}$},
    % ylabel shift = -14pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.02,.5)},rotate=0,anchor=south},
    x label style={yshift=0.3em},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 2, 3, 4, 5, 6, 7, 8, 9, 10},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , , $10^{-2}$ , , , , , , , , ,  , , , , , , , , , $10^{0}$, , , , , , , , , $\mathbf{10^{1}}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=2pt},  % xshift=3pt
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=1e-3,
    ymax=1e1,
    xmin=-20,
    xmax=20,
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    % legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    % legend columns = 8,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend cell align={left},
    legend columns = 4,
    legend style={
      fill opacity=1.0,
      draw opacity=1,
      text opacity=1,
      at={(0.999,0.999)},  % single col: (0.275,0.03) original: (0.91,0.86)
      anchor=north east,
      draw=lightgray,
      font=\scriptsize
    },
    % legend style={
    % cells={anchor=west},
    % % draw=none,
    % fill=none,
    % font=\footnotesize
    % },
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    width=\figwidth,
    height=\figheight,
    scale = \scale
]


% % legend / single row
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(N^{(\text{s},\text{1D})}\)}
% \addplot[very thick, color=violet, solid] coordinates {(0, 1)}; \addlegendentry{\(3\)\hspace{-.5cm}}
% \addplot[very thick, color=teal, solid] coordinates {(0, 1)}; \addlegendentry{\(5\)}
% \addplot[very thick, color=cyan, solid] coordinates {(0, 1)}; \addlegendentry{\(7\)}
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(d^{(\text{s})}\)}
% \addplot[very thick, color=black, solid] coordinates {(0, 1)}; \addlegendentry{\( \lambda/2\)}
% \addplot[very thick, color=black, dashed] coordinates {(0, 1)}; \addlegendentry{\( 3\lambda/2\)}
% \addplot[very thick, color=black, dotted] coordinates {(0, 1)};\addlegendentry{\(2 \lambda\)}


\def\evalstr{"fa_rate"}

\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/Cartesian/X_sweep_same_y/\evalstr.txt};
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/Cartesian/X_sweep_same_y/\evalstr_baseline.txt};
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/Cartesian/X_sweep_same_y/\evalstr_baseline_rad.txt};


\end{semilogyaxis}

\end{tikzpicture}


==> Figures/Cartesian/X_sweep_same_y/precision.tex <==
\begin{tikzpicture}

% \def\scale{.72}  % .72

\begin{semilogyaxis}[
    xlabel={$\mu^{\text{(X)}}$},
    ylabel={$P^\text{(P)}$},
    % ylabel shift = -14pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.02,.5)},rotate=0,anchor=south},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 2, 3, 4, 5, 6},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , ,$10^{-2}$, , , , , , , , ,$10^{-1}$, , , , , , , , , $10^{0}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=2pt},  % xshift=3pt
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=1e-3,
    ymax=1e-0,
    xmin=-30,
    xmax=30,
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    % legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    % legend columns = 8,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend cell align={left},
    legend columns = 4,
    legend style={
      fill opacity=1.0,
      draw opacity=1,
      text opacity=1,
      at={(0.999,0.999)},  % single col: (0.275,0.03) original: (0.91,0.86)
      anchor=north east,
      draw=lightgray,
      font=\scriptsize
    },
    % legend style={
    % cells={anchor=west},
    % % draw=none,
    % fill=none,
    % font=\footnotesize
    % },
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    scale = \scale
]


% % legend / single row
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(N^{(\text{s},\text{1D})}\)}
% \addplot[very thick, color=violet, solid] coordinates {(0, 1)}; \addlegendentry{\(3\)\hspace{-.5cm}}
% \addplot[very thick, color=teal, solid] coordinates {(0, 1)}; \addlegendentry{\(5\)}
% \addplot[very thick, color=cyan, solid] coordinates {(0, 1)}; \addlegendentry{\(7\)}
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(d^{(\text{s})}\)}
% \addplot[very thick, color=black, solid] coordinates {(0, 1)}; \addlegendentry{\( \lambda/2\)}
% \addplot[very thick, color=black, dashed] coordinates {(0, 1)}; \addlegendentry{\( 3\lambda/2\)}
% \addplot[very thick, color=black, dotted] coordinates {(0, 1)};\addlegendentry{\(2 \lambda\)}


\def\evalstr{"precision"}

\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/Cartesian/X_sweep_same_y/\evalstr.txt};
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/Cartesian/X_sweep_same_y/\evalstr_baseline.txt};
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/Cartesian/X_sweep_same_y/\evalstr_baseline_rad.txt};


\end{semilogyaxis}

\end{tikzpicture}


==> Figures/Cartesian/Y_sweep_same_y/f1_score.tex <==
\begin{tikzpicture}

% \def\scale{.72}  % .72

\begin{semilogyaxis}[
    xlabel={y [m]},
    ylabel={$F_1$},
    % ylabel shift = -14pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.02,.5)},rotate=0,anchor=south},
    x label style={yshift=0.3em},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 2, 3, 4, 5, 6},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , ,$10^{-2}$, , , , , , , , , $10^{-1}$ , , , , , , , , , $10^{0}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=2pt},  % xshift=3pt
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=5e-1,
    ymax=1e-0,
    xmin=5,
    xmax=45,
    xtick={5,15,25,35,45},
    xticklabels={$5$,$15$,$25$,$35$,$45$},
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    % legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    % legend columns = 8,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend cell align={left},
    legend columns = 4,
    legend style={
      fill opacity=1.0,
      draw opacity=1,
      text opacity=1,
      at={(0.999,0.999)},  % single col: (0.275,0.03) original: (0.91,0.86)
      anchor=north east,
      draw=lightgray,
      font=\scriptsize
    },
    % legend style={
    % cells={anchor=west},
    % % draw=none,
    % fill=none,
    % font=\footnotesize
    % },
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    width=\figwidth,
    height=\figheight,
    scale = \scale
]


% % legend / single row
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(N^{(\text{s},\text{1D})}\)}
% \addplot[very thick, color=violet, solid] coordinates {(0, 1)}; \addlegendentry{\(3\)\hspace{-.5cm}}
% \addplot[very thick, color=teal, solid] coordinates {(0, 1)}; \addlegendentry{\(5\)}
% \addplot[very thick, color=cyan, solid] coordinates {(0, 1)}; \addlegendentry{\(7\)}
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(d^{(\text{s})}\)}
% \addplot[very thick, color=black, solid] coordinates {(0, 1)}; \addlegendentry{\( \lambda/2\)}
% \addplot[very thick, color=black, dashed] coordinates {(0, 1)}; \addlegendentry{\( 3\lambda/2\)}
% \addplot[very thick, color=black, dotted] coordinates {(0, 1)};\addlegendentry{\(2 \lambda\)}


\def\dirstr{"Cartesian/Y_sweep_same_y"}
\def\evalstr{"f1_score"}

\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr.txt};
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr_baseline.txt};
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr_baseline_rad.txt};


\end{semilogyaxis}

\end{tikzpicture}


==> Figures/Cartesian/Y_sweep_same_y/fa_rate.tex <==
\begin{tikzpicture}

% \def\scale{.72}  % .72

\begin{semilogyaxis}[
    xlabel={y [m]},
    ylabel={$R^\text{(FA)}$},
    % ylabel shift = -14pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.02,.5)},rotate=0,anchor=south},
    x label style={yshift=0.3em},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 2, 3, 4, 5, 6, 7, 8, 9, 10},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , , $10^{-2}$ , , , , , , , , ,  , , , , , , , , , $10^{0}$, , , , , , , , , $\mathbf{10^{1}}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=2pt},  % xshift=3pt
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=1e-3,
    ymax=1e1,
    xmin=5,
    xmax=45,
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    % legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    % legend columns = 8,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend cell align={left},
    legend columns = 4,
    legend style={
      fill opacity=1.0,
      draw opacity=1,
      text opacity=1,
      at={(0.999,0.999)},  % single col: (0.275,0.03) original: (0.91,0.86)
      anchor=north east,
      draw=lightgray,
      font=\scriptsize
    },
    % legend style={
    % cells={anchor=west},
    % % draw=none,
    % fill=none,
    % font=\footnotesize
    % },
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    width=\figwidth,
    height=\figheight,
    scale = \scale
]


% % legend / single row
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(N^{(\text{s},\text{1D})}\)}
% \addplot[very thick, color=violet, solid] coordinates {(0, 1)}; \addlegendentry{\(3\)\hspace{-.5cm}}
% \addplot[very thick, color=teal, solid] coordinates {(0, 1)}; \addlegendentry{\(5\)}
% \addplot[very thick, color=cyan, solid] coordinates {(0, 1)}; \addlegendentry{\(7\)}
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(d^{(\text{s})}\)}
% \addplot[very thick, color=black, solid] coordinates {(0, 1)}; \addlegendentry{\( \lambda/2\)}
% \addplot[very thick, color=black, dashed] coordinates {(0, 1)}; \addlegendentry{\( 3\lambda/2\)}
% \addplot[very thick, color=black, dotted] coordinates {(0, 1)};\addlegendentry{\(2 \lambda\)}


\def\evalstr{"fa_rate"}

\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr.txt};
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr_baseline.txt};
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr_baseline_rad.txt};


\end{semilogyaxis}

\end{tikzpicture}


==> Figures/Cartesian/Y_sweep_same_y/precision.tex <==
\begin{tikzpicture}

% \def\scale{.72}  % .72

\begin{semilogyaxis}[
    xlabel={$a^{\text{(Y)}}$},
    ylabel={$P^\text{(P)}$},
    % ylabel shift = -14pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.02,.5)},rotate=0,anchor=south},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 2, 3, 4, 5, 6},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , ,$10^{-2}$, , , , , , , , ,$10^{-1}$, , , , , , , , , $10^{0}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=2pt},  % xshift=3pt
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=1e-3,
    ymax=1e-0,
    xmin=0,
    xmax=45,
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    % legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    % legend columns = 8,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend cell align={left},
    legend columns = 4,
    legend style={
      fill opacity=1.0,
      draw opacity=1,
      text opacity=1,
      at={(0.999,0.999)},  % single col: (0.275,0.03) original: (0.91,0.86)
      anchor=north east,
      draw=lightgray,
      font=\scriptsize
    },
    % legend style={
    % cells={anchor=west},
    % % draw=none,
    % fill=none,
    % font=\footnotesize
    % },
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    scale = \scale
]



% % legend / single row
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(N^{(\text{s},\text{1D})}\)}
% \addplot[very thick, color=violet, solid] coordinates {(0, 1)}; \addlegendentry{\(3\)\hspace{-.5cm}}
% \addplot[very thick, color=teal, solid] coordinates {(0, 1)}; \addlegendentry{\(5\)}
% \addplot[very thick, color=cyan, solid] coordinates {(0, 1)}; \addlegendentry{\(7\)}
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(d^{(\text{s})}\)}
% \addplot[very thick, color=black, solid] coordinates {(0, 1)}; \addlegendentry{\( \lambda/2\)}
% \addplot[very thick, color=black, dashed] coordinates {(0, 1)}; \addlegendentry{\( 3\lambda/2\)}
% \addplot[very thick, color=black, dotted] coordinates {(0, 1)};\addlegendentry{\(2 \lambda\)}


\def\evalstr{"precision"}

\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr.txt};
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr_baseline.txt};
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr_baseline_rad.txt};


\end{semilogyaxis}

\end{tikzpicture}


==> Figures/Cartesian/Y_sweep_same_y/prob_missed_detect.tex <==

\begin{tikzpicture}[spy using outlines={rectangle, magnification=3.0, size=1.3cm, connect spies}]

% \def\scale{.72}  % .72

\begin{semilogyaxis}[
    xlabel={y [m]},
    ylabel={$P^\text{(MD)}$},
    % ylabel shift = -14pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.02,.5)},rotate=0,anchor=south},
    xlabel style={font=\footnotesize, yshift=0.3em},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 2, 3, 4, 5, 6},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , , $10^{-2}$ , , , , , , , , ,$10^{-1}$, , , , , , , , , $10^{0}$},
    % xtick={5,10,15,20,25,30,35,40,45,50},
    % xticklabels={$5$,$10$, ,$20$, ,$30$, ,$40$, ,$45$},
    yticklabel style={font=\footnotesize,xshift=2pt},  % xshift=3pt
    xticklabel style={font=\footnotesize},
    % xticklabel style={
    %     /pgf/number format/precision=4,
    %     /pgf/number format/fixed, 
    %     font=\footnotesize},
    ymin=1e-3,
    ymax=1e-0,
    xmin=5,
    xmax=45,
    xtick={5,15,25,35,45},
    xticklabels={$5$,$15$,$25$,$35$,$45$},
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    % legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    % legend columns = 8,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend cell align={left},
    legend columns = 3,
    legend style={
      fill opacity=1.0,
      draw opacity=1,
      text opacity=1,
      at={(0.999,0.999)},  % single col: (0.275,0.03) original: (0.91,0.86)
      anchor=north east,
      draw=lightgray,
      font=\scriptsize
    },
    % legend style={
    % cells={anchor=west},
    % % draw=none,
    % fill=none,
    % font=\footnotesize
    % },
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    % mark repeat={2},
    log origin y=infty,
    % set layers=Bowpark, % not working with scope
    legend to name = common_legend,
    width=\figwidth,
    height=\figheight,
    scale = \scale
]

% common legend
\addplot[very thick, color=violet, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{2D Azimuth SARA}
\addplot[very thick, color=teal, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{Baseline \gls{naf}}
\addplot[very thick, color=cyan, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{Baseline Radian}
% \addplot[very thick, color=black, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(d^{(\text{S})} /\lambda = 0.5 \;\)}
% \addplot[very thick, color=black, dashed, draw=none] coordinates {(0, 1)}; \addlegendentry{\(d^{(\text{S})} /\lambda = 1.5 \;\)}
% \addplot[very thick, color=black, dotted, draw=none] coordinates {(0, 1)};\addlegendentry{\(d^{(\text{S})} /\lambda = 2.0\)}

% % legend / single row
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(N^{(\text{s},\text{1D})}\)}
% \addplot[very thick, color=violet, solid] coordinates {(0, 1)}; \addlegendentry{\(3\)\hspace{-.5cm}}
% \addplot[very thick, color=teal, solid] coordinates {(0, 1)}; \addlegendentry{\(5\)}
% \addplot[very thick, color=cyan, solid] coordinates {(0, 1)}; \addlegendentry{\(7\)}
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(d^{(\text{s})}\)}
% \addplot[very thick, color=black, solid] coordinates {(0, 1)}; \addlegendentry{\( \lambda/2\)}
% \addplot[very thick, color=black, dashed] coordinates {(0, 1)}; \addlegendentry{\( 3\lambda/2\)}
% \addplot[very thick, color=black, dotted] coordinates {(0, 1)};\addlegendentry{\(2 \lambda\)}


\def\evalstr{"prob_missed_detect"}

% \addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr.txt};

\addplot[very thick, violet, solid] table [x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr.txt};

% \addplot[very thick, violet, solid, restrict x to domain=0:10, domain=0:10] plot table [x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr_baseline_rad.txt};

% \addplot[very thick, red, solid, restrict x to domain=25:50, domain=25:45] plot table [x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr_baseline_rad.txt};

\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr_baseline.txt};
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr_baseline_rad.txt};

% run 31
% x-start = -5, x_dist=6, x_var=1

\end{semilogyaxis}

% \begin{scope}

%  \spy[gray, on layer=foreground] on (2.85, 2.45) in node [fill=white] at (1.3, 1.3);
% % \spy[gray] on (10.0, 1.0e-2) in node [fill=white] at (30.0, 1.0e-2);

% % \spy[gray] on (3.7, 3.5) in node [fill=white] at (1.0, 2.5);
 
% \end{scope}

\end{tikzpicture}


==> Figures/Cartesian/Y_sweep_same_y/rmse.tex <==
\begin{tikzpicture}

% \def\scale{.72}  % .72

\begin{semilogyaxis}[
    xlabel={y [m]},
    ylabel={$\text{2D NAF RMSE}$},
    % ylabel shift = -14pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.02,.5)},rotate=0,anchor=south},
    x label style={yshift=0.3em},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 2, 3, 4, 5, 6},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , ,  , , , , , , , , ,  , , , , , , , , , $10^{0}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=2pt},  % xshift=3pt
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=1e-3,
    ymax=1e-0,
    xmin=5,
    xmax=45,
    xtick={5,15,25,35,45},
    xticklabels={$5$,$15$,$25$,$35$,$45$},
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    % legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    % legend columns = 8,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend cell align={left},
    legend columns = 4,
    legend style={
      fill opacity=1.0,
      draw opacity=1,
      text opacity=1,
      at={(0.999,0.999)},  % single col: (0.275,0.03) original: (0.91,0.86)
      anchor=north east,
      draw=lightgray,
      font=\scriptsize
    },
    % legend style={
    % cells={anchor=west},
    % % draw=none,
    % fill=none,
    % font=\footnotesize
    % },
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    width=\figwidth,
    height=\figheight,
    scale = \scale
]



% % legend / single row
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(N^{(\text{s},\text{1D})}\)}
% \addplot[very thick, color=violet, solid] coordinates {(0, 1)}; \addlegendentry{\(3\)\hspace{-.5cm}}
% \addplot[very thick, color=teal, solid] coordinates {(0, 1)}; \addlegendentry{\(5\)}
% \addplot[very thick, color=cyan, solid] coordinates {(0, 1)}; \addlegendentry{\(7\)}
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(d^{(\text{s})}\)}
% \addplot[very thick, color=black, solid] coordinates {(0, 1)}; \addlegendentry{\( \lambda/2\)}
% \addplot[very thick, color=black, dashed] coordinates {(0, 1)}; \addlegendentry{\( 3\lambda/2\)}
% \addplot[very thick, color=black, dotted] coordinates {(0, 1)};\addlegendentry{\(2 \lambda\)}


\def\evalstr{"rmse"}

\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr.txt};
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr_baseline.txt};
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/Cartesian/Y_sweep_same_y/\evalstr_baseline_rad.txt};


\end{semilogyaxis}

\end{tikzpicture}


==> Figures/NAF/f1_score.tex <==
\begin{tikzpicture}

% \def\scale{.72}  % .72

\begin{semilogyaxis}[
    xlabel= {$\Delta d^{(\text{P})}$},
    ylabel={$F_1$},
    % ylabel shift = -14pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.02,.5)},rotate=0,anchor=south},
    x label style={yshift=0.3em},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 2, 3, 4, 5, 6},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , ,$10^{-2}$, , , , , , , , , $10^{-1}$ , , , , $\mathbf{5^{-1}}$ , , , , , $10^{0}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=2pt},  % xshift=3pt
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=5e-1,
    ymax=1e-0,
    xmin=0.10,
    xmax=0.17,
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    % legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    % legend columns = 8,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend cell align={left},
    legend columns = 4,
    legend style={
      fill opacity=1.0,
      draw opacity=1,
      text opacity=1,
      at={(0.999,0.999)},  % single col: (0.275,0.03) original: (0.91,0.86)
      anchor=north east,
      draw=lightgray,
      font=\scriptsize
    },
    % legend style={
    % cells={anchor=west},
    % % draw=none,
    % fill=none,
    % font=\footnotesize
    % },
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    width=\figwidth,
    height=\figheight,
    scale = \scale
]


% % legend / single row
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(N^{(\text{s},\text{1D})}\)}
% \addplot[very thick, color=violet, solid] coordinates {(0, 1)}; \addlegendentry{\(3\)\hspace{-.5cm}}
% \addplot[very thick, color=teal, solid] coordinates {(0, 1)}; \addlegendentry{\(5\)}
% \addplot[very thick, color=cyan, solid] coordinates {(0, 1)}; \addlegendentry{\(7\)}
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(d^{(\text{s})}\)}
% \addplot[very thick, color=black, solid] coordinates {(0, 1)}; \addlegendentry{\( \lambda/2\)}
% \addplot[very thick, color=black, dashed] coordinates {(0, 1)}; \addlegendentry{\( 3\lambda/2\)}
% \addplot[very thick, color=black, dotted] coordinates {(0, 1)};\addlegendentry{\(2 \lambda\)}


\def\dirstr{"NAF_sweep"}
\def\evalstr{"f1_score"}

\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr.txt};
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr_baseline.txt};
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr_baseline_rad.txt};


\end{semilogyaxis}

\end{tikzpicture}


==> Figures/NAF/fa_rate.tex <==
\begin{tikzpicture}

% \def\scale{.72}  % .72

\begin{semilogyaxis}[
    xlabel= {$\Delta d^{(\text{P})}$},
    ylabel={$R^\text{(FA)}$},
    % ylabel shift = -14pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.02,.5)},rotate=0,anchor=south},
    x label style={yshift=0.3em},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 2, 3, 4, 5, 6, 7, 8, 9, 10},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , , $10^{-2}$ , , , , , , , , ,$10^{-1}$, , , , , , , , , $10^{0}$, , , , , , , , , $\mathbf{10^{1}}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=2pt},  % xshift=3pt
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=1e-3,
    ymax=1e-0,
    xmin=0.10,
    xmax=0.17,
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    % legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    % legend columns = 8,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend cell align={left},
    legend columns = 4,
    legend style={
      fill opacity=1.0,
      draw opacity=1,
      text opacity=1,
      at={(0.999,0.999)},  % single col: (0.275,0.03) original: (0.91,0.86)
      anchor=north east,
      draw=lightgray,
      font=\scriptsize
    },
    % legend style={
    % cells={anchor=west},
    % % draw=none,
    % fill=none,
    % font=\footnotesize
    % },
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    width=\figwidth,
    height=\figheight,
    scale = \scale
]


% % legend / single row
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(N^{(\text{s},\text{1D})}\)}
% \addplot[very thick, color=violet, solid] coordinates {(0, 1)}; \addlegendentry{\(3\)\hspace{-.5cm}}
% \addplot[very thick, color=teal, solid] coordinates {(0, 1)}; \addlegendentry{\(5\)}
% \addplot[very thick, color=cyan, solid] coordinates {(0, 1)}; \addlegendentry{\(7\)}
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(d^{(\text{s})}\)}
% \addplot[very thick, color=black, solid] coordinates {(0, 1)}; \addlegendentry{\( \lambda/2\)}
% \addplot[very thick, color=black, dashed] coordinates {(0, 1)}; \addlegendentry{\( 3\lambda/2\)}
% \addplot[very thick, color=black, dotted] coordinates {(0, 1)};\addlegendentry{\(2 \lambda\)}


\def\dirstr{"NAF_sweep"}
\def\evalstr{"fa_rate"}

\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr.txt};
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr_baseline.txt};
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr_baseline_rad.txt};



\end{semilogyaxis}

\end{tikzpicture}


==> Figures/NAF/precision.tex <==
\begin{tikzpicture}

% \def\scale{.72}  % .72

\begin{semilogyaxis}[
    xlabel= {$\Delta d^{(\text{P})}$},
    ylabel={$P^\text{(P)}$},
    % ylabel shift = -14pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.02,.5)},rotate=0,anchor=south},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 2, 3, 4, 5, 6},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , ,$10^{-2}$, , , , , , , , ,$10^{-1}$, , , , , , , , , $10^{0}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=2pt},  % xshift=3pt
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=1e-3,
    ymax=1e-0,
    xmin=0.06,
    xmax=0.16,
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    % legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    % legend columns = 8,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend cell align={left},
    legend columns = 4,
    legend style={
      fill opacity=1.0,
      draw opacity=1,
      text opacity=1,
      at={(0.999,0.999)},  % single col: (0.275,0.03) original: (0.91,0.86)
      anchor=north east,
      draw=lightgray,
      font=\scriptsize
    },
    % legend style={
    % cells={anchor=west},
    % % draw=none,
    % fill=none,
    % font=\footnotesize
    % },
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    scale = \scale
]


% % legend / single row
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(N^{(\text{s},\text{1D})}\)}
% \addplot[very thick, color=violet, solid] coordinates {(0, 1)}; \addlegendentry{\(3\)\hspace{-.5cm}}
% \addplot[very thick, color=teal, solid] coordinates {(0, 1)}; \addlegendentry{\(5\)}
% \addplot[very thick, color=cyan, solid] coordinates {(0, 1)}; \addlegendentry{\(7\)}
% \addlegendimage{white, fill=white} % Dummy entry for legend title
% \addlegendentry{\hspace{-.5cm}\(d^{(\text{s})}\)}
% \addplot[very thick, color=black, solid] coordinates {(0, 1)}; \addlegendentry{\( \lambda/2\)}
% \addplot[very thick, color=black, dashed] coordinates {(0, 1)}; \addlegendentry{\( 3\lambda/2\)}
% \addplot[very thick, color=black, dotted] coordinates {(0, 1)};\addlegendentry{\(2 \lambda\)}

\def\dirstr{"NAF_sweep"}
\def\evalstr{"precision"}

\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr.txt};
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr_baseline.txt};
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/\dirstr/\evalstr_baseline_rad.txt};

\end{semilogyaxis}

\end{tikzpicture}


==> Figures/bistatic_setup.tex <==

\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\def \globalscale {1.000000}
\begin{tikzpicture}[y=1pt, x=1pt, inner sep=0pt, outer sep=0pt]

%---------------------------------
\def \axiscolor{black!40}
axis
    \path[draw=white,miter limit=10.0] (15.0, 75.8) -- (37.5, 75.8);
    \path[draw=white,miter limit=10.0] (15.0, 83.2) -- (37.5, 83.2);
    \path[draw=white,miter limit=10.0] (15.0, 90.8) -- (37.5, 90.8);
    \path[draw=white,miter limit=10.0] (15.0, 98.2) -- (37.5, 98.2);
    
    \draw[color=\axiscolor,-{Stealth[scale=1.3,scale width=1.5,color=\axiscolor]}] (7.5, 38.2) -- (67.7, 38.2);
    \node[text=\axiscolor,anchor=south] (text8) at (63.8, 27.8){x}; % near
    
    \draw[color=\axiscolor,-{Stealth[scale=1.3,scale width=1.5,color=\axiscolor]}] (7.5, 38.2) -- (7.5, 98.5);
    \node[text=\axiscolor,anchor=south] (text9) at (3.8, 83.2){z}; % near
    
    \draw[color=\axiscolor,-{Stealth[scale=1.3,scale width=1.5,color=\axiscolor]}] (7.5, 38.2) -- (25.2, 73.7)(27.3, 77.8)(27.3, 77.8) -- (29.0, 81.2)(31.0, 85.3)(31.0, 85.3) -- (32.7, 88.7)(34.8, 92.8)(34.8, 92.8) -- (36.5, 96.2)(38.5, 100.3)(38.5, 100.3) -- (82.4, 187.0);
    \node[text=\axiscolor,anchor=south] (text10) at (72.0, 177.8){y}; % far
    
    \draw[color=\axiscolor,-{Stealth[scale=1.3,scale width=1.5,color=\axiscolor]}] (60.0, 143.2) -- (120.2, 143.2);
    \node[text=\axiscolor,anchor=south] (text16) at (116.2, 132.8){x}; % far
    
    \draw[color=\axiscolor,-{Stealth[scale=1.3,scale width=1.5,color=\axiscolor]}] (60.0, 143.2) -- (60.0, 203.5);
    \node[text=\axiscolor,anchor=south] (text17) at (56.2, 188.2){z}; % far

%---------------------------------
% scatterer operations
    \path[draw=black,fill=violet] (184, 170) ellipse (3pt and 3pt); %circle scatterer
    
    \draw[-{Stealth[scale=1.3,scale width=1.5,color=violet]}] (104.8, 68.2) -- (181.4, 168.7); % arrowline comm->scatterer
    \node[text=violet,anchor=south] (text20) at (150.0, 109.5){\(\mathbf{v}^{(\text{t})}\)};
    \draw[-{Stealth[scale=1.3,scale width=1.5,color=violet]}] (236.0, 68.2) -- (186.4, 168.7); % arrowline sens->scatterer
    \node[text=violet,anchor=south] (text20) at (225.0, 109.5){\(\mathbf{v}^{(\text{r})}\)};
    
    \node[text=violet,anchor=south west,align=center] (text14) at (173, 175){Scatterer \\direction};
    
%---------------------------------
% scan operations
    \draw[-{Stealth[scale=1.3,scale width=1.5,color=teal]}] (104.8, 68.2) -- (143.5, 177.9); %arrowline comm->scan
    \node[text=teal,anchor=south] (text24) at (132.0, 114.0){\(\mathbf{u}^{(\text{t})}\)};
    \draw[-{Stealth[scale=1.3,scale width=1.5,color=teal]}] (236.0, 68.2) -- (243.5, 177.9); %arrowline sens->scan
    \node[text=teal,anchor=south] (text24) at (250.0, 114.0){\(\mathbf{u}^{(\text{r})}\)};
    
    % \node[text=teal,anchor=south west,align=center] (text15) at (128, 184){Scan \\direction};

%---------------------------------
% communications array
    \def \arrayoffset {105.0}
    \def \arraycolor {steelblue31119180}
    \def \arraytext {Transmitter}
    
    \node[text=black,anchor=south,align=center] (text25) at (\arrayoffset, 3){\textcolor{\arraycolor}{\arraytext}\\\textcolor{\arraycolor}{Array}};
    
    \path[draw=\arraycolor,miter limit=10.0] (\arrayoffset+1.2, 27.8) -- (\arrayoffset+1.2, 58.9);
    
    \path[draw=\arraycolor,miter limit=10.0] (\arrayoffset-0.3, 27.8) -- (\arrayoffset-0.3, 58.9);
    
    \path[draw=\arraycolor,fill=white,rounded corners=0.6pt] (\arrayoffset-1.4, 48.8) rectangle 
    (\arrayoffset+2.3, 42.8);
    
    \path[draw=\arraycolor,fill=white,miter limit=10.0] (\arrayoffset-3.7, 53.8) -- (\arrayoffset-11.6, 53.8)
    .. controls (\arrayoffset-16.6, 53.8) and (\arrayoffset-17.9, 56.1) .. (\arrayoffset-15.6, 60.5) -- (\arrayoffset-13.6, 64.4)
    .. controls (\arrayoffset-12.2, 67.0) and (\arrayoffset-9.0, 68.2) .. (\arrayoffset-4.0, 68.2) -- (\arrayoffset+11.7, 68.2)
    .. controls (\arrayoffset+16.7, 68.2) and (\arrayoffset+18.1, 66.0) .. (\arrayoffset+15.8, 61.6) -- (\arrayoffset+13.7, 57.7)
    .. controls (\arrayoffset+12.4, 55.1) and (\arrayoffset+9.2, 53.8) .. (\arrayoffset+4.2, 53.8) -- cycle;

    \path[draw=black,fill=black] (\arrayoffset, 68.2) ellipse (1pt and 1pt);  % black circle 
    
%---------------------------------
% sensing array
    \def \arrayoffset {236.0}
    \def \arraycolor {darkorange25512714}
    \def \arraytext {Receiver}
    
    \node[text=black,anchor=south,align=center] (text25) at (\arrayoffset, 3){\textcolor{\arraycolor}{\arraytext}\\\textcolor{\arraycolor}{Array}};
    
    \path[draw=\arraycolor,miter limit=10.0] (\arrayoffset+1.2, 27.8) -- (\arrayoffset+1.2, 58.9);
    
    \path[draw=\arraycolor,miter limit=10.0] (\arrayoffset-0.3, 27.8) -- (\arrayoffset-0.3, 58.9);
    
    \path[draw=\arraycolor,fill=white,rounded corners=0.6pt] (\arrayoffset-1.4, 48.8) rectangle 
    (\arrayoffset+2.3, 42.8);
    
    \path[draw=\arraycolor,fill=white,miter limit=10.0] (\arrayoffset-3.7, 53.8) -- (\arrayoffset-11.6, 53.8)
    .. controls (\arrayoffset-16.6, 53.8) and (\arrayoffset-17.9, 56.1) .. (\arrayoffset-15.6, 60.5) -- (\arrayoffset-13.6, 64.4)
    .. controls (\arrayoffset-12.2, 67.0) and (\arrayoffset-9.0, 68.2) .. (\arrayoffset-4.0, 68.2) -- (\arrayoffset+11.7, 68.2)
    .. controls (\arrayoffset+16.7, 68.2) and (\arrayoffset+18.1, 66.0) .. (\arrayoffset+15.8, 61.6) -- (\arrayoffset+13.7, 57.7)
    .. controls (\arrayoffset+12.4, 55.1) and (\arrayoffset+9.2, 53.8) .. (\arrayoffset+4.2, 53.8) -- cycle;

    \path[draw=black,fill=black] (\arrayoffset, 68.2) ellipse (1pt and 1pt);  % black circle 
%---------------------------------

\end{tikzpicture}


==> Figures/monostatic_setup.tex <==

\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{steelblue31119180}{RGB}{31,119,180}
% \definecolor{greenmatplot}{RGB}{44,160,44}
% \definecolor{redmatplot}{RGB}{214,39,40}


\def \globalscale {1.000000}
\begin{tikzpicture}[y=1pt, x=1pt, yscale=\globalscale,xscale=\globalscale, every node/.append style={scale=\globalscale}, inner sep=0pt, outer sep=0pt]
  \path[draw=white,miter limit=10.0] (15.0, 75.8) -- (37.5, 75.8);



  \path[draw=white,miter limit=10.0] (15.0, 83.2) -- (37.5, 83.2);



  \path[draw=white,miter limit=10.0] (15.0, 90.8) -- (37.5, 90.8);



  \path[draw=white,miter limit=10.0] (15.0, 98.2) -- (37.5, 98.2);



  \path[draw=black,miter limit=10.0] (7.5, 38.2) -- (62.7, 38.2);



  \path[draw=black,fill=black,miter limit=10.0] (66.7, 38.2) -- (61.4, 35.6) -- 
  (62.7, 38.2) -- (61.4, 40.9) -- cycle;



  \path[draw=black,miter limit=10.0] (7.5, 38.2) -- (7.5, 93.5);



  \path[draw=black,fill=black,miter limit=10.0] (7.5, 97.4) -- (10.1, 92.2) -- 
  (7.5, 93.5) -- (4.9, 92.2) -- cycle;



  \path (60.0, 38.2) rectangle (67.5, 23.2);



  \begin{scope}[shift={(-0.4, 0.4)}]
    \node[text=black,anchor=south] (text8) at (63.8, 27.8){x};



  \end{scope}
  \path (0.0, 98.2) rectangle (7.5, 83.2);



  \begin{scope}[shift={(-0.4, 0.4)}]
    \node[text=black,anchor=south] (text9) at (3.8, 83.2){z};



  \end{scope}
  \path[draw=black,miter limit=10.0] (7.5, 38.2) -- (25.2, 73.7)(27.3, 
  77.8)(27.3, 77.8) -- (29.0, 81.2)(31.0, 85.3)(31.0, 85.3) -- (32.7, 
  88.7)(34.8, 92.8)(34.8, 92.8) -- (36.5, 96.2)(38.5, 100.3)(38.5, 100.3) -- 
  (80.4, 184.0);



  \path[draw=black,fill=black,miter limit=10.0] (82.1, 187.5) -- (82.1, 181.6) 
  -- (80.4, 184.0) -- (77.4, 184.0) -- cycle;



  \begin{scope}[shift={(-0.4, 0.4)}]
    \node[text=black,anchor=south] (text10) at (72.0, 177.8){y};



  \end{scope}
  \path[draw=black,miter limit=10.0] (60.0, 143.2) -- (115.2, 143.2);



  \path[draw=black,fill=black,miter limit=10.0] (119.2, 143.2) -- (113.9, 140.6)
   -- (115.2, 143.2) -- (113.9, 145.9) -- cycle;



  \path[draw=black,miter limit=10.0] (60.0, 143.2) -- (60.0, 198.5);



  \path[draw=black,fill=black,miter limit=10.0] (60.0, 202.4) -- (62.6, 197.2) 
  -- (60.0, 198.5) -- (57.4, 197.2) -- cycle;



  \path[draw=black,fill=violet] (184, 170) ellipse (3pt and 3pt); %circle scatterer



  \begin{scope}[shift={(-0.4, 0.4)}]
    \node[text=violet,anchor=south west,align=center] (text14) at (173, 175){Scatterer \\direction};



  \end{scope}
  % \path[draw=black,fill=white] (143.2, 170) ellipse (3pt and 3pt); %circle scan

  \path[draw=black,fill=black] (123.8, 68.2) ellipse (1pt and 1pt); %circle panels



  \begin{scope}[shift={(-0.4, 0.4)}]
    \node[text=teal,anchor=south west,align=center] (text15) at (128, 184){Scan \\direction};



  \end{scope}
  \path (112.5, 143.2) rectangle (120.0, 128.2);



  \begin{scope}[shift={(-0.4, 0.4)}]
    \node[text=black,anchor=south] (text16) at (116.2, 132.8){x};



  \end{scope}
  \path (52.5, 203.2) rectangle (60.0, 188.2);



  \begin{scope}[shift={(-0.4, 0.4)}]
    \node[text=black,anchor=south] (text17) at (56.2, 188.2){z};



  \end{scope}
  % \draw[draw=black,dashed,miter limit=10.0] (123.8, 68.2) -- (192.4, 176.7);



  % \path[draw=black,fill=black,miter limit=10.0] (194.5, 180.0) -- (194.0, 
  % 174.2) -- (192.4, 176.7) -- (189.5, 177.0) -- cycle;



  \draw[draw=black,miter limit=10.0] (123.8, 68.2) -- (180.4, 163.7); % arrowline scatterer



  \path[draw=violet,fill=violet,miter limit=10.0] (182.5, 167.0) -- (182.0, 
  161.2) -- (180.4, 163.7) -- (177.5, 164.0) -- cycle; % arrowhead scatterer



  \begin{scope}[shift={(-0.4, 0.4)}]
    \node[text=violet,anchor=south] (text20) at (160.0, 109.5){\(\mathbf{v}\)};



  \end{scope}
  % \path[draw=teal,miter limit=10.0] (123.8, 68.2) -- (141.6, 161.1);



  % \path[draw=teal,fill=teal,miter limit=10.0] (142.3, 164.9) -- (143.9, 
  % 159.3) -- (141.6, 161.1) -- (138.8, 160.3) -- cycle;



  \path[draw=black,miter limit=10.0] (123.8, 68.2) -- (143.5, 177.9); %arrowline scan



  \path[draw=teal,fill=teal,miter limit=10.0] (144.3, 181.9) -- (145.9, 
  176.3) -- (143.6, 178.1) -- (140.8, 177.3) -- cycle; %arrowhead scan



  \begin{scope}[shift={(-0.4, 0.4)}]
    \node[text=teal,anchor=south] (text24) at (138.8, 114.0){\(\mathbf{u}\)};



  \end{scope}
  \path (74.2, 30.8) rectangle (164.2, 0.8);



%---------------------------------
% communications array
    \def \arrayoffset {104.0}
    \def \arraycolor {steelblue31119180}
    \def \arraytext {Transmitter}
    
    % \node[text=black,anchor=south,align=center] (text25) at (\arrayoffset, 3){\textcolor{\arraycolor}{\arraytext}\\\textcolor{\arraycolor}{Array}};
    
    \path[draw=\arraycolor,miter limit=10.0] (\arrayoffset+1.2, 27.8) -- (\arrayoffset+1.2, 58.9);
    
    \path[draw=\arraycolor,miter limit=10.0] (\arrayoffset-0.3, 27.8) -- (\arrayoffset-0.3, 58.9);
    
    \path[draw=\arraycolor,fill=white,rounded corners=0.6pt] (\arrayoffset-1.4, 48.8) rectangle 
    (\arrayoffset+2.3, 42.8);
    
    \path[draw=\arraycolor,fill=white,miter limit=10.0] (\arrayoffset-3.7, 53.8) -- (\arrayoffset-11.6, 53.8)
    .. controls (\arrayoffset-16.6, 53.8) and (\arrayoffset-17.9, 56.1) .. (\arrayoffset-15.6, 60.5) -- (\arrayoffset-13.6, 64.4)
    .. controls (\arrayoffset-12.2, 67.0) and (\arrayoffset-9.0, 68.2) .. (\arrayoffset-4.0, 68.2) -- (\arrayoffset+11.7, 68.2)
    .. controls (\arrayoffset+16.7, 68.2) and (\arrayoffset+18.1, 66.0) .. (\arrayoffset+15.8, 61.6) -- (\arrayoffset+13.7, 57.7)
    .. controls (\arrayoffset+12.4, 55.1) and (\arrayoffset+9.2, 53.8) .. (\arrayoffset+4.2, 53.8) -- cycle;

%---------------------------------
% sensing array
    \def \arrayoffset {137.0}
    \def \arraycolor {darkorange25512714}
    \def \arraytext {Receiver}
    
    % \node[text=black,anchor=south,align=center] (text25) at (\arrayoffset, 3){\textcolor{\arraycolor}{\arraytext}\\\textcolor{\arraycolor}{Array}};
    
    \path[draw=\arraycolor,miter limit=10.0] (\arrayoffset+1.2, 27.8) -- (\arrayoffset+1.2, 58.9);
    
    \path[draw=\arraycolor,miter limit=10.0] (\arrayoffset-0.3, 27.8) -- (\arrayoffset-0.3, 58.9);
    
    \path[draw=\arraycolor,fill=white,rounded corners=0.6pt] (\arrayoffset-1.4, 48.8) rectangle 
    (\arrayoffset+2.3, 42.8);
    
    \path[draw=\arraycolor,fill=white,miter limit=10.0] (\arrayoffset-3.7, 53.8) -- (\arrayoffset-11.6, 53.8)
    .. controls (\arrayoffset-16.6, 53.8) and (\arrayoffset-17.9, 56.1) .. (\arrayoffset-15.6, 60.5) -- (\arrayoffset-13.6, 64.4)
    .. controls (\arrayoffset-12.2, 67.0) and (\arrayoffset-9.0, 68.2) .. (\arrayoffset-4.0, 68.2) -- (\arrayoffset+11.7, 68.2)
    .. controls (\arrayoffset+16.7, 68.2) and (\arrayoffset+18.1, 66.0) .. (\arrayoffset+15.8, 61.6) -- (\arrayoffset+13.7, 57.7)
    .. controls (\arrayoffset+12.4, 55.1) and (\arrayoffset+9.2, 53.8) .. (\arrayoffset+4.2, 53.8) -- cycle;

%---------------------------------
% array text
    \node[text=black,anchor=south,align=center] (text25) at (116, 3){\textcolor{steelblue31119180}{Transmitter} + \textcolor{darkorange25512714}{Receiver}\\Co-located Arrays};
    
%---------------------------------
% monostatic box
  \draw[draw=black, rounded corners=5pt, dashed] (85.0, 50.0) rectangle ++(72.0, 22.0);
  % \node[text=black,anchor=south west,align=center] (textsumco) at (160.0, 57.0){Sum Co-Array};
  \node[text=black,anchor=south west,align=left] (textsumco) at (160.0, 50.0){Monostatic \\Setup};


\end{tikzpicture}

